Dynamics: A different outlook

The present article deals with general mechanics in an unconventional manner. At first, Newtonian mechanics for a point particle has been described in vectorial picture, considering Cartesian, polar and tangent-normal formulations in a unified manner. An extensive differential geometric notions have been used when motion on curved surfaces has been considered. Both the Lagrangian and the Hamiltonian formulations have been discussed with various examples. The relevant part of the calculus of variation has been presented in the appendix. Also, a detailed study about the nature of the Lagrangian has been shown in the appendix and it has been found that the usual Lagrangian can be extended to curved space-time using the notion of differential geometry. The article may be suitable both for undergraduate and postgraduate students.

==> Chapter1/chapter1.tex <==
\chapter{Preliminary}

~~~\textbf{Result I:} If $\vec{a}(t)$ is a vector of constant magnitude i.e. $|\vec{a}(t)|=$ constant, then $\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}t}$ is orthogonal to $\vec{a}$.

\textbf{Proof:} As $|\vec{a}(t)|=$ constant,

So, $\vec{a}\cdot\vec{a}=|\vec{a}|^2=$ constant

$\therefore ~2\vec{a}\cdot\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}t}=0$

Hence for non-zero vector $\vec{a}$,  $\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}t}$ is orthogonal to $\vec{a}$.\\

\textbf{Remark:} A natural question arises for a unit vector :

If $\vec{a}$ is an unit vector then $\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}t}$ is orthogonal to $\vec{a}$. But does $\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}t}$ is also an unit vector?\\

\textbf{Result II:} If $\vec{a}$ is an unit vector then $\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}\theta}$ is an unit vector.

\begin{wrapfigure}[8]{r}{0.48\textwidth}
	\includegraphics[height=4.5 cm , width=7 cm ]{f1.pdf}
	\begin{center}
		Fig. 1.1
	\end{center}\vspace{-\intextsep}
\end{wrapfigure}

\textbf{Proof:}  Let $\overrightarrow{OP}=\vec{a}$ be the position of the unit vector in time $t$ and $\overrightarrow{OQ}$ be the position of the unit vector in time $t+\Delta t$. As $\vec{a}$ is a unit vector, so, $OP=OQ=1$.

Let $\angle POQ=\Delta\theta$.  Draw $ON\perp PQ$.

Let $\overrightarrow{OQ}=\vec{a}+\overrightarrow{\Delta a}$,  so that $\overrightarrow{PQ}=\overrightarrow{\Delta a}$ and $\overrightarrow{NQ}=\dfrac{1}{2}\overrightarrow{\Delta a}$.

Now, in $\triangle ONQ$, ~$\dfrac{NQ}{OQ}=\sin\left(\dfrac{1}{2}\Delta\theta\right)$

$\therefore~\sin\left(\dfrac{1}{2}\Delta\theta\right)=NQ=|\overrightarrow{NQ}|=\dfrac{1}{2}|\overrightarrow{\Delta a}|$

$\therefore~\dfrac{\sin\left(\dfrac{1}{2}\Delta\theta\right)}{\dfrac{1}{2}\Delta\theta}=\dfrac{\dfrac{1}{2}|\overrightarrow{\Delta a}|}{\dfrac{1}{2}\Delta\theta}$

Now proceed to the limit as $\Delta\theta\rightarrow0$, we have $\big|\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}\theta}=1\big|$.

Hence $\dfrac{\mathrm{d}\vec{a}}{\mathrm{d}\theta}$ is perpendicular to $\vec{a}$ and is of unit magnitude.

